RoBin: Facilitating the Reproduction of Configuration-Related Vulnerability

Vulnerability reproduction paves a way in debugging software failures, which need intensive manual efforts. However, some key factors (e.g., software configuration, trigger method) are often missing, so we can not directly reproduce the failure without extra attempts. Even worse, highly customized configuration options of programs create a barrier for reproducing the vulnerabilities that only appear under some specific combinations of configurations. In this paper, we address the problem mentioned above -- reproducing the configuration-related vulnerability. We try to solve it by proposing a binary similarity-based method to infer the specific building configurations via the binary from crash report. The main challenges are as follows: precise compilation option inference, program configuration inference, and source-code-to-binary matching. To achieve the goal, we implement RoBin, a binary similarity-based building configuration inference tool. To demonstrate the effectiveness, we test RoBin on 21 vulnerable cases upon 4 well-known open-source programs. It shows a strong ability in pinpointing the building configurations causing the vulnerability. The result can help developers reproduce and diagnose the vulnerability, and finally, patch the programs.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\para{Data segments in the crash dump} In our approach, we leverage code segments in the crash dump as our input to figure out the building configurations needed in the software building process. But in the crash dump, there are not only the code segments but also data segments(\eg .data, .bss, heap, stack regions). In order to fully take advantage of the crash dump, we will explore the possibility to leverage data segments to figure out the building configurations, which could lead to our further research. For now, we have some useful rules to infer building configurations from data segments:

\begin{itemize}
    \item The definition of some data structures are controlled by configurations;
    \item The size of some data structures are decided by some configurations;
    \item The existence of some fields in the data structures could be identified by concrete values.
\end{itemize}

%\para{\fixme{False Positive in the tool chain}} IDA Pro and BinDiff

%\para{\fixme{Signatures for binary matching}} More matching rules to get

\para{More algorithms for Binary Code Similarity} Although BinDiff is the state-of-art industry tool, which diffs binary code, we would like to integrity more approaches(\eg Deep Learning~\cite{10.1145/3133956.3134018}) to calculate binary code similarity. We believe those tools could combine and complement the limitations of each other to give us a more precise binary code similarity result.

==> impl.tex <==
\section{Implementation}
\label{sec:impl}
We implement \sys with about 3k lines of Python code. Equipped with several commercial tools (\eg IDA Pro\cite{disassembler2010debugger}, BinDiff\cite{bindiff}), we can establish the whole system.

Binary comparison leverages BinDiff, the most modern commercial tool in the industry field. Bindiff helps to analyze the similarity of different binaries by constructing the graph of binaries with the help of $networkx$ package of Python. It greatly helps the process of compilation options inference. During the recursive binary generation, it will come out with a confidence result indicating the degree of similarity between the generated binary and crash report binary.

Source code feature extraction and macro relation analysis are mainly based on Typechef\cite{typechef}, which can analyze the relationship between macros in the source code. The analysis procedure needs to obtain whether the function is related to the macro and the function existence condition (what constraints need to be met by the function existence), Typechef does not directly provide the interface. So we analyze the definition of VAST nodes in TypeChef and customize an interface to accomplish the source code feature extraction.

We leverage IDA Pro, the most advanced tool in the industry, to extract the binary feature, which serves as a disassembler. When extracting binary features, we use $networkx$ package of Python to encapsulate the data from IDA Pro. For the instructions in the binary, only the key instructions, such as $cmp$, $string$, $constant$, etc., are kept, and the remaining instructions are removed. The reserved instructions are recombined to the original graph structure, which can be used for the matching procedure.

At last, we utilize the Python interface $Z3$ for constraint solving. To make it easier to solve the constraints, we convert the macro expressions and the expressions into a recognizable form for the solver.



